StageDesigner: Artistic Stage Generation for Scenography via Theater Scripts

In this work, we introduce StageDesigner, the first comprehensive framework for artistic stage generation using large language models combined with layout-controlled diffusion models. Given the professional requirements of stage scenography, StageDesigner simulates the workflows of seasoned artists to generate immersive 3D stage scenes. Specifically, our approach is divided into three primary modules: Script Analysis, which extracts thematic and spatial cues from input scripts; Foreground Generation, which constructs and arranges essential 3D objects; and Background Generation, which produces a harmonious background aligned with the narrative atmosphere and maintains spatial coherence by managing occlusions between foreground and background elements. Furthermore, we introduce the StagePro-V1 dataset, a dedicated dataset with 276 unique stage scenes spanning different historical styles and annotated with scripts, images, and detailed 3D layouts, specifically tailored for this task. Finally, evaluations using both standard and newly proposed metrics, along with extensive user studies, demonstrate the effectiveness of StageDesigner. Project can be found at: https://deadsmither5.github.io/2025/01/03/StageDesigner/

==> sec/7.application.tex <==
\section{Application Scenarios}

The StageDesigner system offers valuable applications for both general users and professional stage designers.
\smallbreak
\noindent \textbf{For General Users:} StageDesigner enables users without design training to create visually engaging and thematically aligned stage layouts from basic text input. By feeding the final generated result back to the LLM, users can make conversational edits to refine and experiment with 3D scene setups, exploring narrative visualization and scenographic interpretations. This accessibility is especially useful for theater enthusiasts, educators, and students, offering an engaging way to understand thematic staging.
\smallbreak
\noindent \textbf{For Professional Stage Designers:} StageDesigner enhances professional workflows by enabling rapid exploration of scene concepts, saving time during initial design and revisions. By generating cohesive layouts directly from scripts, the system supports designers in experimenting with thematic variations and quickly iterating on design choices. The Script Analysis Module ensures all elements align with the narrative and atmosphere, helping designers effectively capture the script’s essence. Moreover, StageDesigner-generated 3D models can be imported into software like Blender for further customization, offering professionals a flexible starting point that integrates with their tools. 
